Two-dimensional Quantum Gravity

This Ph.D. thesis pursues two goals: The study of the geometrical structure of two-dimensional quantum gravity and in particular its fractal nature. To address these questions we review the continuum formalism of quantum gravity with special focus on the scaling properties of the theory. We discuss several concepts of fractal dimensions which characterize the extrinsic and intrinsic geometry of quantum gravity. This work is partly based on work done in collaboration with Jan Ambj{\o}rn, Dimitrij Boulatov, Jakob L. Nielsen and Yoshiyuki Watabiki (1997). The other goal is the discussion of the discretization of quantum gravity and to address the so called quantum failure of Regge calculus. We review dynamical triangulations and show that it agrees with the continuum theory in two dimensions. Then we discuss Regge calculus and prove that a continuum limit cannot be taken in a sensible way and that it does not reproduce continuum results. This work is partly based on work done in collaboration with Jan Ambj{\o}rn, Jakob L. Nielsen and George Savvidy (1997).

==> FIGURES/solution.tex <==
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(6462,4839)(751,-4288)
\thicklines
\put(1201,-3961){\vector( 0, 1){4500}}
\put(1201,-3961){\vector( 1, 0){6000}}
\put(1201,-2761){\line( 1, 0){1800}}
\put(3076,-2761){\line( 0,-1){1200}}
\put(3076,-4261){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}lab1}}}
\put(6601,-4261){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}lab3}}}
\put(751, 89){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}lab4}}}
\put(751,-2836){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}lab2}}}
\end{picture}

